Critical initialisation for deep signal propagation in noisy rectifier neural networks

Stochastic regularisation is an important weapon in the arsenal of a deep learning practitioner. However, despite recent theoretical advances, our understanding of how noise influences signal propagation in deep neural networks remains limited. By extending recent work based on mean field theory, we develop a new framework for signal propagation in stochastic regularised neural networks. Our noisy signal propagation theory can incorporate several common noise distributions, including additive and multiplicative Gaussian noise as well as dropout. We use this framework to investigate initialisation strategies for noisy ReLU networks. We show that no critical initialisation strategy exists using additive noise, with signal propagation exploding regardless of the selected noise distribution. For multiplicative noise (e.g. dropout), we identify alternative critical initialisation strategies that depend on the second moment of the noise distribution. Simulations and experiments on real-world data confirm that our proposed initialisation is able to stably propagate signals in deep networks, while using an initialisation disregarding noise fails to do so. Furthermore, we analyse correlation dynamics between inputs. Stronger noise regularisation is shown to reduce the depth to which discriminatory information about the inputs to a noisy ReLU network is able to propagate, even when initialised at criticality. We support our theoretical predictions for these trainable depths with simulations, as well as with experiments on MNIST and CIFAR-10

==> other.tex <==
\section{Introduction}

Deep neural networks have been at the centre of some of the most impressive recent successes in machine learning. Furthermore, advances in network design have reduced the burden of training such large neural models as well as helped to prevent overfitting. These advances include improved weight initialization strategies~\citep{glorot2010understanding, he2015delving}, non-saturating activation functions~\citep{glorot2011deep} and stochastic regularization techniques~\citep{srivastava2014dropout}. 

%\textcolor{red}{TODO: explain the following prior work....} Specifically, \citet{glorot2010understanding} proposed the Xavier initialization. \citet{glorot2011deep} prosed the ReLU activation function. The weight initialisation for ReLU was then proposed by \citet{he2015delving}. To regularize network \citet{srivastava2014dropout} proposed dropout corresponding to Bernoulli noise. However, injecting other types of noise such as Gaussian or Poisson have also been showed to improve the performance of deep models \citep{poole2014analyzing}. 

However, despite these advances our theoretical understanding of how these combined mechanisms affect neural networks remain impoverished. In particular, we are interested in the following research questions: How is signal propagation in deep neural networks affected by noise? And to what extend do current weight initialization strategies, when combined with noise induced regularization, maintain their beneficial properties? \textcolor{red}{TODO: chat about deep information propagation work} 

To answer these questions, we begin by extending the mean field framework developed by \citet{poole2016exponential} to describe noisy signal propagation for common noise distributions, such as those selected from the exponential family. Although this extended framework can support arbitrary nonlinearities, we focus on rectifier neural networks with ReLU activation, arguably the most popular activation function used in practice. \textcolor{red}{TODO: describe what we did in the paper...}

In the following section we briefly describe the framework developed by \cite{poole2016exponential} and in the next section extend this theoretical framework to be able to describe noise injected signal propagation dynamics.

\section{Review of signal propagation in deep neural networks}

Given input $\mathbf{x}^0 \in \mathbb{R}^{D_0}$, consider the following deep neural network model 
\begin{align}
	\mathbf{h}^l = W^l\mathbf{x}^{l-1} + \mathbf{b}^l,
	\label{eq: deep model} 
\end{align}
where the hidden layer activations $\mathbf{x}^l = \phi(\mathbf{h}^l)$ are computed element-wise using an activation function $\phi(\cdot)$ with weights $W^l \in \mathbb{R}^{D_l \times D_{l-1}}$ and biases $\mathbf{b}^l \in \mathbb{R}^{D_l}$, for $l = 1, ..., L$. Here, $D_l$ denotes the dimensionality of the $l^{th}$ hidden layer in the network. The elements for the weights and biases are sampled i.i.d. from a zero mean Gaussian distribution with variance $\sigma^2_w/D_{l-1}$ and $\sigma^2_b$, respectively. The variance of each weight is scaled according to the incoming hidden layer dimensionality to ensure that the activity per neuron remains independent of the number of neurons connected to it in the previous layer. Using an argument based on self-averaging, valid in the limiting case for large width networks, \citet{poole2016exponential} showed that the empirical distribution of the pre-activations $\mathbf{h}^l$ can be treated as being Gaussian distributed with mean zero and variance 
\begin{align}
	q^l = \sigma^2_w \int \mathcal{D}_z \phi\left(\sqrt{q^{l-1}}z \right)^2 + \sigma^2_b,
	\label{eq: variance map}
\end{align}
with $\mathcal{D}_z = \frac{dz}{\sqrt{2\pi}}e^{-\frac{z^2}{2}}$ and initial value $q^0 = \frac{1}{D^0}\mathbf{x}^0\cdot\mathbf{x}^0$. The recursive relation in~\eqref{eq: variance map} serves as an iterative map that can be used to compute the variance of the pre-activations at each layer. This iterative map is displayed in Figure  for a tanh network (green curve). 

A desirable property to encourage information to flow through the network is for the pre-activations $\mathbf{h}^l$ to have roughly constant variance across layers during signal propagation. In the context of the above framework, this property is satisfied everywhere by a length map trajectory that corresponds to the identity line, shown as a dashed black line in Figure . Therefore, a fixed point (representing constant variance) for an arbitrary trajectory exists only where its curve intersects the identity line. This fixed point is then described by the following relation
\begin{align}
	q^* = \sigma^2_w \int \mathcal{D}_z \phi\left(\sqrt{q^* z} \right)^2 + \sigma^2_b.
	\label{eq: variance map fixed point}
\end{align}
In the next section we extend this mean field framework for noisy neural network signal propagation, capable of providing dynamics for a general class of noise distributions. 

\section{Noisy signal propagation}

%To understand how noise influences signal propagation in a random network, we begin by considering the model $\tilde{\mathbf{h}}^l = W^l\tilde{\mathbf{x}}^{l-1} + \mathbf{b}^l$, where $\tilde{\mathbf{x}}^{l}$ is a corrupted version of $\mathbf{x}^l = \phi(\tilde{\mathbf{h}}^l)$. To corrupt each input $\mathbf{x}^l$ we specify a noise distribution 
%\begin{align*}
%  p(\tilde{\mathbf{x}}^l | \mathbf{x}^l) = \prod^D_{j=1}\textrm{P}(\tilde{\mathbf{x}}^l_j| \mathbf{x}^l_j, \gamma^l_j),
%\end{align*}
%where $\tilde{\mathbf{x}}^l$ represents the inputs at layer $l$ with added noise. The distribution over the corrupted inputs is assumed to factor over the input dimension and we assume that $\textrm{E}(\tilde{x}^l_j) = x^l_j, \forall j \in D$, such that $\textrm{E}[\tilde{\mathbf{x}}^l] = \mathbf{x}^l$. For example, at each layer $l$, we can select a noise distribution from the exponential family given the natural parameters $\gamma^l_j$ and the original input component $\mathbf{x}^l_j$. 

To understand how noise influences signal propagation in a random network, we inject noise into the model using the operator~$\odot$ to denote either addition or multiplication and define a noisy version of the model in (\ref{eq: deep model}) as
\begin{align}
	\tilde{\mathbf{h}}^l = W^l(\mathbf{x}^{l-1}\odot \epsilon^{l-1}) + \mathbf{b}^l,
	\label{eq: noisy deep model}
\end{align}
where $\epsilon^l$ is a vector of hidden activation noise, sampled from a pre-specified noise distribution. \textcolor{red}{TODO: mention more complicated case?} The model defined in (\ref{eq: noisy deep model}) therefore allows for the injection of noise at different levels of the network including the input, hidden units as well as hidden activations. This gives the second moment of the empirical distribution of inputs at layer $l$ as
\begin{align*}
	\tilde{q}^l = \frac{1}{D_l}\sum^{D_l}_{j=1}(\tilde{\mathbf{h}}^l_j)^2,
\end{align*}
%Let $\tilde{\mathbf{x}}^l = \mathbf{x}^l \odot \epsilon^{l-1}_\mathbf{x}$, then in expectation over the weights, biases and noise distribution
which in expectation over the weights, biases and noise distribution becomes
\begin{align*}
	\tilde{q}^l & = \textrm{E}_{\mathbf{w}, \mathbf{b}, \epsilon}[(\tilde{\mathbf{h}}^l_j)^2] \\ & = \textrm{E}_{\mathbf{w}, \epsilon}[\{\mathbf{w}^{l,j}\cdot (\mathbf{x}^{l-1}_j \odot \epsilon^{l-1}_j)\}^2] + \textrm{E}_{\mathbf{b}}[(\mathbf{b}^l_j)^2] \\
	& = \sigma^2_{w}\frac{1}{D_{l-1}}\sum^{D_{l-1}}_{j=1} \left [ \phi(\tilde{\mathbf{h}}^{l-1}_{j})^2 \odot \textrm{E}[(\epsilon^{l-1}_j)^2] \right ] + \sigma^2_b.
\end{align*}
Using the same self-averaging argument as in \citet{poole2016exponential}, we assume (in the large width limit) that the empirical distribution of noisy inputs across the hidden units of a \textit{fixed} network, converges to the distribution of noisy inputs to a single hidden unit, across different \textit{random} networks. In doing so, we can replace the above average of the inputs with an integral over a standard Gaussian random variable and use the observation that the previous pre-activation layer is assumed to be Gaussian distributed with mean zero and variance $\tilde{q}^{l-1}$. This gives the following noisy variance map
\begin{align}
	\tilde{q}^l = \sigma^2_w (\tilde{\eta}^{l-1} \odot \mu^{l-1}_2) + \sigma^2_b,
	\label{eq: noisy variance relation}
\end{align}
where $\tilde{\eta}^l = \Phi \left (\phi \left (\sqrt{\tilde{q}^lz} \right)^2 \right)$ with $\Phi(f(z)) = \int \mathcal{D}_z f(z)$ and $\mu^l_2 = \textrm{E}[(\epsilon^{l})^2]$. Table \ref{tab: noise table} provides special cases of this recursive variance relation for several common noise distributions. For example, in the case of additive Gaussian noise with mean zero and variance $\sigma^2_\epsilon$, the relation in \eqref{eq: noisy variance relation} becomes $\tilde{q}^l = \sigma^2_w (\tilde{\eta}^{l-1} +  \sigma^2_\epsilon) + \sigma^2_b$. \textcolor{red}{TODO: Explain Figure 1}. In the following section, we use equation \eqref{eq: noisy variance relation} to derive critical initialization strategies for ReLU networks.

\begin{figure}
 \includegraphics[width=\linewidth]{figs/add_noise.pdf}
 \caption{\textit{Noisy signal propagation}. Lines correspond to theoretical predictions and points to numerical simulations, for random tanh networks with no noise (purple), tanh networks with additive Gaussian noise with $\sigma^2_\epsilon = 1$ (yellow), ReLU networks with no noise (green) and ReLU networks with additive Gaussian noise with $\sigma^2_\epsilon = 1$ (blue). \textbf{Left}:~Iterative variance map where the identity line is displayed as a dashed black line. \textbf{Right}:~Growth in variance during forward signal propagation.}
 \label{fig:boat1}
\end{figure}

% Our interest is in understanding how noise influences signal propagation in a random network. To inject noise into the model, similar to {}\citep{poole2014analyzing} we use the operator~$\odot$ to denote either addition or multiplication and define a noisy version of the model in (\ref{eq: deep model}) as
% \begin{align}
% 	\tilde{\mathbf{h}}^l = (W^l\mathbf{x}^{l-1}\odot \epsilon^{l-1}_\mathbf{x} + \mathbf{b}^l)\odot \epsilon^l_\mathbf{h},
% 	\label{eq: noisy deep model}
% \end{align}
% where $\epsilon^l_\mathbf{x}$ is a vector of hidden activation noise and $\epsilon^l_\mathbf{h}$ is noise injected into the hidden units at layer $l$, sampled from a pre-specified noise distribution. The model defined in (\ref{eq: noisy deep model}) therefore allows for the injection of noise at different levels of the network including the input, hidden units as well as hidden activations.   

%\subsection{Adding noise to the input of each layer of the network}

%Consider $\tilde{\mathbf{h}}^l = W^l\tilde{\mathbf{x}}^{l-1} + \mathbf{b}^l$, where $\tilde{\mathbf{x}}^{l}$ is a corrupted version of $\mathbf{x}^l$. To corrupt each input $\mathbf{x}^l$ we specify a noise distribution 
%\begin{align}
%  p(\tilde{\mathbf{x}}^l | \mathbf{x}^l) = \prod^D_{j=1}P(\tilde{\mathbf{x}}^l_j| \mathbf{x}^l_j, \eta^l_j),
%  \label{eq: noise dist}
%\end{align}
%where $\tilde{\mathbf{x}}^l$ represents the inputs at layer $l$ with added noise. The distribution over the corrupted inputs is assumed to factor over the input dimension. For example, a distribution from the exponential family given the natural parameters $\eta_j$ and the original input component $\mathbf{x}_j$. Then

%A common form of noise injected learning is to add noise to the inputs $\mathbf{h}^l_j$, for each layer of the network. 

\begin{table}[t]
\caption{Noisy variance maps for common noise distributions.}
\label{tab: noise table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llll}
\toprule
 Distribution & $\textrm{p}(\epsilon)$ & $\mu_2$ & Variance map \\
\toprule
--- Additive Noise ---  \\
\midrule
Gaussian & $\mathcal{N}(0, \sigma^2_\epsilon) $ & $\sigma^2_\epsilon$ \vspace{0.5em} & $\tilde{q}^l = \sigma^2_w (\tilde{\eta}^{l-1} +  \sigma^2_\epsilon) + \sigma^2_b$\\
Laplace  & $Lap(0, \beta)$ & $2\beta^2$ \vspace{0.5em} & $\tilde{q}^l = \sigma^2_w (\tilde{\eta}^{l-1} +  2\beta^2) + \sigma^2_b $\\
\toprule
 --- Multiplicative Noise ---  \\
\midrule
Gaussian & $\mathcal{N}(1, \sigma^2_\epsilon) $ & $(\sigma^2_\epsilon + 1)$ \vspace{0.5em} & $\tilde{q}^l = \sigma^2_w \left [ \tilde{\eta}^{l-1}(\sigma^2_\epsilon + 1)\right ] + \sigma^2_b$\\
Laplace  & $Lap(1, \beta)$ & $(2\beta^2 + 1)$ \vspace{0.5em} & $\tilde{q}^l = \sigma^2_w \left [\tilde{\eta}^{l-1}(2\beta^2 + 1)\right ] + \sigma^2_b $\\
Poisson  & $Pois(1)$ & $2$ \vspace{0.5em} & $\tilde{q}^l = 2\sigma^2_w \tilde{\eta}^{l-1} + \sigma^2_b $\\
%Bernoulli & $Bern(p)$ & $p$ \vspace{0.5em} & $\tilde{q}^l = p\sigma^2_w\tilde{\eta}^{l-1} + \sigma^2_b $\\
Dropout   & \makecell[l]{$\textrm{p}(\epsilon = \frac{1}{p}) = p,$\\$\textrm{p}(\epsilon = 0) = 1-p$ } & $\frac{1}{p}$ \vspace{0.5em} & $\tilde{q}^l = \frac{\sigma^2_w} {p} \tilde{\eta}^{l-1} + \sigma^2_b$\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

% \begin{table}[t]
% \caption{Marginalised noise from exponential family distributions.}
% \label{tab: noise table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{llll}
% \toprule
% Distribution & $P(\tilde{\mathbf{x}}_j | \mathbf{x}_j, \gamma_j)$ & $\textrm{Var}(\tilde{\mathbf{x}}_j)$ & $\tilde{q}^l$ \\
% \midrule
% Bernoulli & $Bern(\mathbf{x}_j, p)$ & $\frac{1-p}{p}\mathbf{x}^2_j$ \vspace{0.5em} & $\frac{\sigma^2_w}{p}\tilde{\eta}^{l-1} + \sigma^2_b $\\
% Gaussian & $\mathcal{N}(\mathbf{x}_j, \sigma^2_\epsilon) $ & $\sigma^2_\epsilon$ \vspace{0.5em} & $\sigma^2_w (\tilde{\eta}^{l-1} +  \sigma^2_\epsilon) + \sigma^2_b$\\
% Laplace  & $Lap(\mathbf{x}_j, \lambda)$ & $2\lambda^2$ \vspace{0.5em} & $\sigma^2_w (\tilde{\eta}^{l-1} +  2\lambda^2) + \sigma^2_b $\\
% Poisson   & $Pois(\mathbf{x}_j)$ & $\mathbf{x}_j$ \vspace{0.5em} & $\sigma^2_w \left [ \tilde{\eta}^{l-1} + \Phi \left (\phi \left (\sqrt{\tilde{q}^{l-1}}z \right) \right) \right ] + \sigma^2_b$\\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}


% \subsection{Adding noise at different levels of the network}

% A slightly more involved strategy is to add noise at different stages of the network, for example at both the hidden units as well as the hidden activations. For simplicity, we only consider the bias-free regime. Using a first order Taylor expansion as in \citep{bishop1995training} for small noise (which ensures that the contribution of higher order terms are negligible), we have that
% \begin{align}
% 	\phi(W^l\tilde{\mathbf{x}}^{l-1} + \epsilon^l_\mathbf{h}) \approx \phi(W^l\tilde{\mathbf{x}}^{l-1}) + \textrm{diag}(\phi^{\prime}(W^l\tilde{\mathbf{x}}^{l-1}))\epsilon^l_\mathbf{h},
% 	\label{eq: taylor expansion}
% \end{align} 
% where we use the operator $\textrm{diag}(\mathbf{z})$ to denote a diagonal matrix with the elements of $\mathbf{z}$ on the diagonal and here $\tilde{\mathbf{x}}^l = \mathbf{x}^{l} + \epsilon^{l}_\mathbf{x}$. Therefore, adding noise to the hidden units at layer $l$ is approximately equivalent to adding a scaled version of the noise to the hidden activations. If the input noise is chosen to be Gaussian with a specified covariance such that $\epsilon^0_\mathbf{x} \sim \mathcal{N}(0, \Sigma)$, it can be shown that this is also equivalent to adding noise of the form $\epsilon^1_\mathbf{h} \sim \mathcal{N}(0, W^1\Sigma{W^1}^T)$, to the units in first hidden layer of the network. Furthermore, using the result in (\ref{eq: taylor expansion}), we can now condense all the different forms of noise into a sampled noise vector $\epsilon^1_\mathbf{x} \sim \mathcal{N}(0, \textrm{diag}(\phi^{\prime}(W^1\mathbf{x}^{0}))W^1\Sigma{W^1}^T)$ injected into the activations of the first hidden layer~\citep{poole2014analyzing}. Continuing with the same reasoning, we can define the following approximate recursive relation %, provided that the singular values of $W^1$ are sufficiently small (for more detail see Section ...)
% \begin{align}
% 	\tilde{\mathbf{h}}^l \approx W^l(\phi(\tilde{\mathbf{h}}^{l-1}) + \epsilon_\mathbf{x}^{l-1}), 
% \end{align}
% where $\epsilon^l_\mathbf{x} \sim \mathcal{N}(0, \Sigma^l)$, $\Sigma^l = A^lW^l\Sigma^{l-1}{W^l}^T$ and $A^l = \textrm{diag}(\phi^{\prime}(W^l\mathbf{x}^{l-1}))$.

% Now for noisy neural networks...
% \begin{align}
% 	\tilde{q}^l_\mathcal{A} & = \textrm{E}_{\mathbf{w}, \epsilon}[\{\mathbf{w}^{l,j}\cdot(\phi(\tilde{\mathbf{h}}^{l-1}) + \epsilon^{l-1}_{\mathbf{x}})\}^2] \\
% 	& = \sigma^2_{w}\frac{1}{D_{l-1}}\sum^{D_{l-1}}_{i=1} \phi(\tilde{\mathbf{h}}^{l-1}_{i})^2 + \textrm{Var}(\mathbf{w}^{l,j}\cdot \epsilon^{l-1}_{\mathbf{x}}) 
% \end{align}

%where 
%
%\begin{align}
%	\textrm{Var}(\mathbf{w}^{l,j} \cdot \epsilon^{l-1}_\mathbf{x}) & = \textrm{Var}\left(\sum^{D_{l-1}}_{i=1}\mathbf{w}^{l,j}_i \epsilon^{l-1}_{\mathbf{x}, i} \right) \\
%	& = \sum^{D_{l-1}}_{i=1}\textrm{Var}\left(\mathbf{w}^{l,j}_i \epsilon^{l-1}_{\mathbf{x}, i} \right) + 2\sum^{D_{l-1}-1}_{i=1}\sum^{D_{l-1}}_{k=i+1}\textrm{Cov}(\mathbf{w}^{l,j}_i \epsilon^{l-1}_{\mathbf{x}, i}, \mathbf{w}^{l,j}_k \epsilon^{l-1}_{\mathbf{x}, k}) \\
%\end{align}
%
%\begin{align}
%	\textrm{Var}(\mathbf{w}^{l,j} \cdot \epsilon^{l-1}_\mathbf{x}) & = \textrm{Var}\left(\sum^{D_{l-1}}_{i=1}\mathbf{w}^{l,j}_i \epsilon^{l-1}_{\mathbf{x}, i} \right) \\
%	& = \sum^{D_{l-1}}_{i=1}\textrm{Var}\left(\mathbf{w}^{l,j}_i \epsilon^{l-1}_{\mathbf{x}, i} \right) + 2\sum^{D_{l-1}-1}_{i=1}\sum^{D_{l-1}}_{k=i+1}\textrm{Cov}(\mathbf{w}^{l,j}_i \epsilon^{l-1}_{\mathbf{x}, i}, \mathbf{w}^{l,j}_k \epsilon^{l-1}_{\mathbf{x}, k}) \\
%\end{align}
%
%now
%\begin{align}
%	\textrm{Var}\left(\mathbf{w}^{l,j}_i \epsilon^{l}_{\mathbf{x}, i} \right) & = \textrm{Var}(\mathbf{w}^{l,j}_i)\textrm{E}(\epsilon^{l-1}_{\mathbf{x}, i})^2+\textrm{Var}(\epsilon^{l-1}_{\mathbf{x}, i})\textrm{E}(\mathbf{w}^{l,j}_i)^2+\textrm{Var}(\mathbf{w}^{l,j}_i)\textrm{Var}(\epsilon^{l-1}_{\mathbf{x}, i}) \\
%	& = \frac{\sigma^2_w(\sigma^{l-1}_{\epsilon,i})^2}{D_{l-1}}
%\end{align}
%where $(\sigma^{l}_{\epsilon,i})^2 = \phi^{\prime}(\mathbf{h}^{l}_i)\sum^{D_{l-1}}_{j=1}\sigma^2_w(\sigma^{l-1}_{\epsilon,j})^2/D_{l-1}$ and
%\begin{align}
%	\textrm{Cov}(\mathbf{w}^{l,j}_i \epsilon^{l}_{\mathbf{x}, i}, \mathbf{w}^{l,j}_k \epsilon^{l}_{\mathbf{x}, k}) & = \textrm{Cov}(\mathbf{w}^{l,j}_i, \mathbf{w}^{l,j}_k)\textrm{E}(\epsilon^{l}_{\mathbf{x}, i})\textrm{E}(\epsilon^{l}_{\mathbf{x}, k}) \\ & \textcolor{white}{spa} +\textrm{Cov}(\epsilon^{l}_{\mathbf{x}, i}, \epsilon^{l}_{\mathbf{x}, k})\textrm{E}(\mathbf{w}^{l,j}_i)\textrm{E}(\mathbf{w}^{l,j}_k) \\ & \textcolor{white}{space} +\textrm{Cov}(\mathbf{w}^{l,j}_i, \mathbf{w}^{l,j}_k)\textrm{Cov}(\epsilon^{l}_{\mathbf{x}, i}, \epsilon^{l}_{\mathbf{x}, k}) \\
%	& = 0
%\end{align}


% which in the supplementary material is shown to be equal to
% \begin{align}
% 	\tilde{q}^l_\mathcal{A} & = \sigma^2_{w}\frac{1}{D_{l-1}} \sum^{D_{l-1}}_{j=1} \left [ \phi(\tilde{\mathbf{h}}^{l-1}_j)^2 + (\sigma^{l-1}_{\epsilon,j})^2 \right ],
% \end{align}
% where $(\sigma^{l}_{\epsilon,i})^2 = \phi^{\prime}(\mathbf{h}^{l}_i)\sum^{D_{l-1}}_{j=1}\sigma^2_w(\sigma^{l-1}_{\epsilon,j})^2/D_{l-1}$. 
% Now, if we assume a pre-specified diagonal isotropic covariance, i.e. $\Sigma^0 = \textrm{diag}((\sigma^0_\epsilon)^2)$, we get that 
% \begin{align}
% 	\tilde{q}^l_\mathcal{A} & = \sigma^2_{w}\frac{1}{D_{l-1}} \sum^{D_{l-1}}_{j=1} \left [ \phi(\tilde{\mathbf{h}}^{l-1}_j)^2 + \phi^{\prime}(\mathbf{h}^{l-1}_j)\sigma^2_w(\sigma^{l-2}_\epsilon)^2 \right ]
% \end{align}
% and thus we get the following iterative variance map
% \begin{align}
% 	\tilde{q}^l_\mathcal{A} = \sigma^2_{w} \left [ \Phi \left (\phi \left (\sqrt{\tilde{q}_\mathcal{A}^{l-1}}z \right)^2 \right) + \Phi \left (\phi^{\prime}\left(\sqrt{q^{l-1}}z\right) \right)\sigma^2_w(\sigma^{l-2}_\epsilon)^2 \right ].
% \end{align}
% Note that the initial state of the iterative variance map begins with $\tilde{q}^1_\mathcal{A} = q^1 = \sigma^2_wq^0$.

%\subsection{Correlation dynamics for noisy networks}

\section{Critical initialization for noisy rectifier networks}

The success of a particular initialization strategy strongly depends on its ability to initialize at the critical fixed point variance. This helps to ensure that in the forward pass information can continue to flow through the network, unimpeded by adverse signal propagation dynamics that cause the signal to either explode, or vanish. For noisy ReLU networks, this fixed point relation is given by
\begin{align*}
	\tilde{q}^* & = \sigma^2_w \left [ \int^\infty_{-\infty} \mathcal{D}_z \phi\left(\sqrt{\tilde{q}^*}z \right)^2 \odot \mu_2 \right ] + \sigma^2_b \\ 
	& = \sigma^2_w \left [ \left (\int^0_{-\infty} \mathcal{D}_z \phi\left(\sqrt{\tilde{q}^*}z \right)^2 + \int^{\infty}_0 \mathcal{D}_z \phi\left(\sqrt{\tilde{q}^*}z \right)^2 \right ) \odot \mu_2 \right ] + \sigma^2_b,
\end{align*}
where the signal over the negative domain gets clamped such that
\begin{align}
	\tilde{q}^* & = \sigma^2_w \left [\tilde{q}^* \int^{\infty}_0 \mathcal{D}_z z^2 \odot \mu_2 \right ] + \sigma^2_b \nonumber \\
	& = \sigma^2_w\left (\frac{1}{2}\tilde{q}^* \odot \mu_2 \right) + \sigma^2_b. 
	\label{eq: crit init relu}
\end{align}
Therefore, a critical initialization for a noisy ReLU network corresponds to a function of the tuple $(\sigma_w, \sigma_b, \mu_2)$, that satisfies the recursion relation in \eqref{eq: crit init relu}. The existence of such a solution strongly depends on the type of noise that is being injected into the network. In the case of additive noise, $\tilde{q}^* = \sigma^2_w\frac{1}{2}\tilde{q}^* + \mu_2 \sigma^2_w + \sigma^2_b$, which implies that the only critical point initialization is given by $(\sigma_w, \sigma_b, \mu_2) = (\sqrt{2}, 0, 0)$. Therefore, any amount of additive noise from a distribution with mean zero and non-zero variance will destroy the critical point. However, for multiplicative noise, $\tilde{q}^* = \sigma^2_w\frac{1}{2}\tilde{q}^*\mu_2 + \sigma^2_b$, and the solution $(\sigma_w, \sigma_b, \mu_2) = \left ( \sqrt{\frac{2}{\mu_2}}, 0, \mu_2 \right)$ provides a critical initialization for noise distributions with a mean equal to one and a non-zero second moment~$\mu_2$. For example, in the case of dropout noise $\mu_2 = 1/p$, such that to initialization at criticality $(\sigma_w, \sigma_b) = (\sqrt{2p}, 0)$. Furthermore, for multiplicative Gaussian noise, $\mu_2 = \sigma^2_\epsilon + 1$ and we find that $(\sigma_w, \sigma_b) = (\sqrt{\frac{2}{\sigma^2 + 1}}, 0)$. \textcolor{red}{TODO: Explain Figure 2}. For a summary of critical initializations for commonly used noise distributions see Table \ref{tab: crit init table}. 

\begin{table}[t]
\caption{Critical point initialization for noisy ReLU networks.}
\label{tab: crit init table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lll}
\toprule
Distribution & Fixed point map & critical point initialization \\
\toprule
--- Additive Noise ---  \\
\midrule
Gaussian & $\tilde{q}^* = \sigma^2_w\frac{1}{2}\tilde{q}^* + \sigma^2_w\sigma^2_\epsilon + \sigma^2_b$ & $(\sigma_w, \sigma_b, \sigma_\epsilon) = (\sqrt{2}, 0, 0)$ \\
Laplace  & $\tilde{q}^* = \sigma^2_w\frac{1}{2}\tilde{q}^* + 2\sigma^2_w\beta^2 + \sigma^2_b$ & $(\sigma_w, \sigma_b, \beta) = (\sqrt{2}, 0, 0)$ \\
\toprule
--- Multiplicative Noise ---  \\
\midrule
Gaussian & $\tilde{q}^* = \sigma^2_w\frac{1}{2}\tilde{q}^*(\sigma^2_\epsilon+1) + \sigma^2_b$ & $(\sigma_w, \sigma_b, \sigma_\epsilon) = \left ( \sqrt{\frac{2}{\sigma^2_\epsilon+1}}, 0, \sigma_\epsilon \right)$ \\
Laplace  & $\tilde{q}^* = \sigma^2_w\frac{1}{2}\tilde{q}^*(2\beta^2 + 1) + \sigma^2_b$ & $(\sigma_w, \sigma_b, \beta) = \left(\sqrt{\frac{2}{2\beta^2 + 1}}, 0, \beta \right)$ \\
Poisson   & $\tilde{q}^* = \sigma^2_w\tilde{q}^* + \sigma^2_b$ & $(\sigma_w, \sigma_b, \lambda) = \left(1, 0, 1 \right)$ \\
%Bernoulli & $\tilde{q}^* = p\sigma^2_w\frac{1}{2}\tilde{q}^* + \sigma^2_b$ &  $(\sigma_w, \sigma_b, p) = (\sqrt{\frac{2}{p}}, 0, p)$ \\
Dropout & $\tilde{q}^* = \frac{\sigma^2_w}{p}\frac{1}{2}\tilde{q}^* + \sigma^2_b$ &  $(\sigma_w, \sigma_b, p) = (\sqrt{2p}, 0, p)$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}
 \includegraphics[width=\linewidth]{figs/mult_noise.pdf}
 \caption{\textit{Critical initialization for ReLU networks with dropout.} Lines correspond to theoretical predictions and points to numerical simulations, for random ReLU networks with dropout ($p = 0.8$), initialized according to the method proposed by \citet{he2015delving} (purple) and at criticality (yellow). \textbf{Left}:~Iterative variance map where the identity line is displayed as a dashed black line. \textbf{Right}:~Growth in variance during forward signal propagation.}
 \label{fig:boat1}
\end{figure}

% \subsection{Gaussian noise}

% For additive Gaussian noise the relation in \eqref{eq: crit init relu} becomes $\tilde{q}^* = \sigma^2_w\frac{1}{2}\tilde{q}^* + \sigma^2_w\sigma^2_\epsilon + \sigma^2_b$, giving the only critical point as $(\sigma_w, \sigma_b, \sigma_e) = (\sqrt{2}, 0, 0)$ (since the variances must all be non-negative). This implies that any amount of additive Gaussian noise will destroy the existence of a critical point initialization for a ReLU network. An analogous derivation can easily be performed for the case of additive Laplace noise with a similar conclusion. 

%\subsection{Poisson noise}

%In the case of Poisson noise with rate parameter $\lambda = 1$, the second moment is simply equal to $2$ and therefore $\tilde{q}^* = \sigma^2_w\tilde{q}^* + \sigma^2_b$. Therefore again, any amount of noise ensures that no critical point exists.


% \subsection{Dropout noise}

% Dropout is arguably the most popular stochastic regularization technique used in practice and works by multiplying a scaled version of Bernoulli noise with the inputs of a network. For dropout noise, the recursive relation in \eqref{eq: crit init relu} becomes
% \begin{align*}
% 	\tilde{q}^* = \frac{\sigma^2_w}{p}\frac{1}{2}\tilde{q}^* + \sigma^2_b.
% \end{align*}
% which results in a set of critical solutions $(\sigma_w, \sigma_b, p) = (\sqrt{2p}, 0, p)$, dependent on the dropout rate $0 < p \leq 1$. \textcolor{red}{TODO: explain dropout experiments}.

% \subsection{Additive vs. multiplicative noise}

% The fundamental difference between the existence of a set of critical solutions between the difference types of noise is whether the noise is additive or multiplicative. For example, even though additive Gaussian noise removes all critical solutions, it is easy to show that multiplicative Gaussian noise 



\section{Gradient backpropagation in noisy rectifier networks}

Recent work by \citet{schoenholz2016deep} showed that an important factor responsible for reliable gradient flow during backpropagation is $\tilde{\chi} = \sigma^2_w \int \mathcal{D}_z\phi^{\prime}\left(\sqrt{\tilde{q}^*}z\right)^2$, which also happens to be related to the mean squared singular values of the input-output Jacobian $\mathbf{J} = \prod^L_{l=1} \textrm{diag}(\phi^\prime(\tilde{\mathbf{h}}^l))W^l$. Furthermore, during backpropagation, the expected magnitude of the gradient at each layer was shown to be proportional to the variance of its error vector $\tilde{\delta}^l$ and the following recursive variance relation was derived\footnote{An important note is that the derivation relies on the assumption that the weights used in the forward pass are sampled independently from those used during backpropagation.} 
\begin{align}
	\tilde{q}^l_\delta = \tilde{q}^{l+1}_\delta\frac{D_{l+1}}{D_l}\tilde{\chi},
	\label{eq: error variance relation}
\end{align}
where $\tilde{q}^l_\delta = \textrm{E}[(\tilde{\delta}^l_i)^2]$ with $\tilde{\delta}^l_i = \phi^\prime(\tilde{h}^l_i)\sum^{D_{l+1}}_{j=1}\tilde{\delta}^{l+1}_jW^{l+1}_{ji}$. For a network using ReLU activation $\int \mathcal{D}_z\phi^{\prime}\left(\sqrt{\tilde{q}^*}z\right)^2 = \int_0^\infty \mathcal{D}_z = \frac{1}{2}$, independent of the fixed point $\tilde{q}^*$ and therefore, $\tilde{\chi} = \frac{1}{2}\sigma^2_w$. In the case of constant width networks, the fixed point for \eqref{eq: error variance relation} requires that $\tilde{\chi} = 1$ such that $\sigma^2_w = 2$. However, critical initialization for multiplicative noise implies that $\tilde{\chi} = \frac{1}{2}\left(\sqrt{\frac{2}{\mu_2}}\right)^2 = \frac{1}{\mu_2}$. Therefore, to satisfy the relation in \eqref{eq: error variance relation}, the network architecture must adapt to the amount of noise injected into the network in such a way that the layer width $D_{l+1} = \mu_2D_l$. For example, in the case of dropout $D_{l+1} = D_l/p$, which implies that for any $p < 1$, each successive layer in the network needs to grow in width by a factor of $1/p$ to promote stable gradient flow. Similarly, for multiplicative Gaussian noise, $D_{l+1} = D_l(\sigma^2_\epsilon + 1)$, which requires the network to grow in width unless $\sigma^2_\epsilon = 0$.

\textcolor{red}{TODO: discuss experiments}

% The correlation dynamic for noisy neural networks are given by

% \begin{align}{}
% 	\tilde{q}^l_{ab} = \frac{1}{D_l}\sum^{D_l}_{j=1}\tilde{h}^l_j(\mathbf{x}^{0,a})\tilde{h}^l_j(\mathbf{x}^{0,b})
% \end{align}

% \begin{align}
% 	\tilde{q}^l_{ab} = \sigma^2_w\frac{1}{D_{l-1}}\sum^{D_{l-1}}_{j=1}\phi(\tilde{h}^{l-1}_j(\mathbf{x}^{0,a}))\phi(\tilde{h}^{l-1}_j(\mathbf{x}^{0,b})) + \sigma^2_b
% \end{align}
% Let $\tilde{\mathbf{x}}^{l-1, a} = \phi(\tilde{h}^{l-1}_j(\mathbf{x}^{0,a}))$, since the noise is sampled independently we then have that $\textrm{E}_\epsilon \left [ \tilde{\mathbf{x}}^{l-1, a} \cdot \tilde{\mathbf{x}}^{l-1, b} \right ] = \textrm{E}_\epsilon \left [ \tilde{\mathbf{x}}^{l-1, a} \right ] \cdot \textrm{E}_\epsilon \left [ \tilde{\mathbf{x}}^{l-1, b} \right ] = \mathbf{x}^{l-1, a} \cdot \mathbf{x}^{l-1, b}$. Using the result derived in \citep{poole2016exponential} we have

% \begin{align*}
% 	\tilde{q}^l_{ab} = \sigma^2_w \int \mathcal{D}_{z_1}\mathcal{D}_{z_2}\phi(\tilde{u}_1)\phi(\tilde{u}_2) + \sigma^2_b,
% \end{align*}
% where $\tilde{u}_1 = \sqrt{\tilde{q}^{l-1}_{aa}}z_1$ and $\tilde{u}_2 = \sqrt{\tilde{q}^{l-1}_{bb}}\left (\tilde{c}^{l-1}_{ab}z_1 + \sqrt{1-(\tilde{c}^{l-1}_{ab})^2}z_2 \right )$ with $\tilde{c}^l_{ab} = \frac{\tilde{q}^{l}_{ab}}{\sqrt{\tilde{q}^l_{aa}}\sqrt{\tilde{q}^l_{bb}}}$.


% Dynamical isometry in dropout rectifier networks

% In our case the mean squared singular value of the Jacobian is $\tilde{\chi}^L$, where 
% \begin{align}
% 	%\tilde{\chi} = \frac{\partial \tilde{c}^l_{ab}}{\partial \tilde{c}^{l-1}_{ab}} = \sigma^2_w \int \mathcal{D}_z\phi^{\prime}\left(\sqrt{\tilde{q}^*}z\right)^2
% 	\tilde{\chi} = \sigma^2_w \int \mathcal{D}_z\phi^{\prime}\left(\sqrt{\tilde{q}^*}z\right)^2
% 	\label{eq: chi}
% \end{align}
% thus we require that $\tilde{\chi} = 1$. For ReLU network $\int \mathcal{D}_z\phi^{\prime}\left(\sqrt{\tilde{q}^*}z\right)^2 = \int_0^\infty \mathcal{D}_z = \frac{1}{2}$, independent of the fixed point variance $\tilde{q}^*$. Therefore, $\chi = \frac{1}{2}\sigma^2_w$ which implies that $\sigma^2_w = 2$. 

% Furthermore, similar to ... it is relatively easy to show that if $\tilde{c}^{l-1}_{ab} = 1$ with $\tilde{q}_{aa} = \tilde{q}_{bb} = \tilde{q}^*$, then
% \begin{align*}
% 	\tilde{c}^l_{ab} & = \frac{\tilde{q}^l_{ab}}{\tilde{q}^*} \\
% 	& = \frac{1}{\tilde{q}^*}\left [ \sigma^2_w \int \mathcal{D}_z \phi(\sqrt{\tilde{q}^*}z)^2 + \sigma^2_b \right ] \\
% 	& = \frac{1}{\tilde{q}^*}\left [ \tilde{q}^* - \sigma^2_w\textrm{Var}(\tilde{\mathbf{x}}) \right ] \\
% 	& = 1 - \frac{\sigma^2_w\textrm{Var}(\tilde{\mathbf{x}})}{\tilde{q}^*},
% \end{align*}
% which in fact holds for any nonlinearity.

% For example, dropout satisfies the fixed point of recursive variance relation when $\sigma_w = \sqrt{2p}$, however this means that
% \begin{align*}
% 	\tilde{\chi} = \left (\sqrt{2p} \right)^2\frac{1}{2} = p
% \end{align*}
% which for any amount of dropout implies that $\chi < 1$.

\section{Experiments}

\section{Discussion}

In practice, a dropout rate of $p = 0.5$ has often been found to work well for ReLU networks \citep{srivastava2014dropout}. Interestingly, the critical initialization corresponding to this rate is $(\sigma_w, \sigma_b) = (\sqrt{2p}, 0) = (1, 0)$. This is exactly the ``Xavier'' initialization proposed by \citet{glorot2010understanding}, which prior to the method developed in \cite{he2015delving}, was often used in combination with dropout \cite{simonyan2014very}. This could therefore help to explain the initial success associated with this specific dropout rate. Similarly, \citet{srivastava2014dropout} reported that adding multiplicative Gaussian noise where $\epsilon \sim \mathcal{N}(1, \sigma^2_\epsilon)$, with $\sigma^2_\epsilon = 1$, also seemed to perform well, for which the critical initialization is $\left ( \sqrt{\frac{2}{\sigma^2_\epsilon+1}}, 0 \right) = (1, 0)$, again corresponding to the ``Xavier'' method.

\textcolor{red}{TODO: explain dynamical isometry}

Using tools of free probability \citet{pennington2017resurrecting} were able to derive the first two moments of the spectral density of $\mathbf{JJ}^T$ for a random constant width ReLU network as $m_1 = \left (\sigma^2_w/2 \right)^L$ and $m_2 = \left(\sigma^2_w/2\right)^{2L}(2L + 1)$. In our context, initializing at criticality for multiplicative noise distributions then gives the corresponding mean as $m_1 = (1/\mu_2)^L$, and variance as $\sigma^2_{JJ^T} = m_2 - m_1^2 = 2L\left(1/\mu_2 \right)^{2L}$. Therefore, for constant width, large depth noisy ReLU networks, the mean of the spectral density will either explode, or vanish, unless $\mu_2 = 1$. However, for all the common multiplicative noise distributions in Table \ref{tab: noise table}, any amount of noise results in $\mu_2 > 1$. For example, for dropout $\mu_2 = 1$ only if $1/p = 1$, which implies that $p=1$. For Gaussian noise it is required that $\sigma^2_\epsilon + 1 = 1$, such that $\sigma^2_\epsilon$ must be zero. Therefore noise, even at criticality, results in a vanishing mean. Similarly, $\sigma^2_{JJ^T}$ will also vanish for large $L$, when $\mu_2 > 1$.

%\section{Submission of papers to NIPS 2018}
%
%NIPS requires electronic submissions.  The electronic submission site
%is
%\begin{center}
%  \url{https://cmt.research.microsoft.com/NIPS2018/}
%\end{center}
%
%Please read the instructions below carefully and follow them faithfully.
%
%\subsection{Style}
%
%Papers to be submitted to NIPS 2018 must be prepared according to the
%instructions presented here. Papers may only be up to eight pages
%long, including figures. Additional pages \emph{containing only
%  acknowledgments and/or cited references} are allowed. Papers that
%exceed eight pages of content (ignoring references) will not be
%reviewed, or in any other way considered for presentation at the
%conference.
%
%The margins in 2018 are the same as since 2007, which allow for
%$\sim$$15\%$ more words in the paper compared to earlier years.
%
%Authors are required to use the NIPS \LaTeX{} style files obtainable
%at the NIPS website as indicated below. Please make sure you use the
%current files and not previous versions. Tweaking the style files may
%be grounds for rejection.
%
%\subsection{Retrieval of style files}
%
%The style files for NIPS and other conference information are
%available on the World Wide Web at
%\begin{center}
%  \url{http://www.nips.cc/}
%\end{center}
%The file \verb+nips_2018.pdf+ contains these instructions and
%illustrates the various formatting requirements your NIPS paper must
%satisfy.
%
%The only supported style file for NIPS 2018 is \verb+nips_2018.sty+,
%rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{}
%  2.09, Microsoft Word, and RTF are no longer supported!}
%
%The \LaTeX{} style file contains three optional arguments: \verb+final+,
%which creates a camera-ready copy, \verb+preprint+, which creates a
%preprint for submission to, e.g., arXiv, and \verb+nonatbib+, which will
%not load the \verb+natbib+ package for you in case of package clash.
%
%\paragraph{New preprint option for 2018}
%If you wish to post a preprint of your work online, e.g., on arXiv,
%using the NIPS style, please use the \verb+preprint+ option. This will
%create a nonanonymized version of your work with the text
%``Preprint. Work in progress.''  in the footer. This version may be
%distributed as you see fit. Please \textbf{do not} use the
%\verb+final+ option, which should \textbf{only} be used for papers
%accepted to NIPS.
%
%At submission time, please omit the \verb+final+ and \verb+preprint+
%options. This will anonymize your submission and add line numbers to aid
%review. Please do \emph{not} refer to these line numbers in your paper
%as they will be removed during generation of camera-ready copies.
%
%The file \verb+nips_2018.tex+ may be used as a ``shell'' for writing
%your paper. All you have to do is replace the author, title, abstract,
%and text of the paper with your own.
%
%The formatting instructions contained in these style files are
%summarized in Sections \ref{gen_inst}, \ref{headings}, and
%\ref{others} below.
%
%\section{General formatting instructions}
%\label{gen_inst}
%
%The text must be confined within a rectangle 5.5~inches (33~picas)
%wide and 9~inches (54~picas) long. The left margin is 1.5~inch
%(9~picas).  Use 10~point type with a vertical spacing (leading) of
%11~points.  Times New Roman is the preferred typeface throughout, and
%will be selected for you by default.  Paragraphs are separated by
%\nicefrac{1}{2}~line space (5.5 points), with no indentation.
%
%The paper title should be 17~point, initial caps/lower case, bold,
%centered between two horizontal rules. The top rule should be 4~points
%thick and the bottom rule should be 1~point thick. Allow
%\nicefrac{1}{4}~inch space above and below the title to rules. All
%pages should start at 1~inch (6~picas) from the top of the page.
%
%For the final version, authors' names are set in boldface, and each
%name is centered above the corresponding address. The lead author's
%name is to be listed first (left-most), and the co-authors' names (if
%different address) are set to follow. If there is only one co-author,
%list both author and co-author side by side.
%
%Please pay special attention to the instructions in Section \ref{others}
%regarding figures, tables, acknowledgments, and references.
%
%\section{Headings: first level}
%\label{headings}
%
%All headings should be lower case (except for first word and proper
%nouns), flush left, and bold.
%
%First-level headings should be in 12-point type.
%
%\subsection{Headings: second level}
%
%Second-level headings should be in 10-point type.
%
%\subsubsection{Headings: third level}
%
%Third-level headings should be in 10-point type.
%
%\paragraph{Paragraphs}
%
%There is also a \verb+\paragraph+ command available, which sets the
%heading in bold, flush left, and inline with the text, with the
%heading followed by 1\,em of space.
%
%\section{Citations, figures, tables, references}
%\label{others}
%
%These instructions apply to everyone.
%
%\subsection{Citations within the text}
%
%The \verb+natbib+ package will be loaded for you by default.
%Citations may be author/year or numeric, as long as you maintain
%internal consistency.  As to the format of the references themselves,
%any style is acceptable as long as it is used consistently.
%
%The documentation for \verb+natbib+ may be found at
%\begin{center}
%  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
%\end{center}
%Of note is the command \verb+\citet+, which produces citations
%appropriate for use in inline text.  For example,
%\begin{verbatim}
%   \citet{hasselmo} investigated\dots
%\end{verbatim}
%produces
%\begin{quote}
%  Hasselmo, et al.\ (1995) investigated\dots
%\end{quote}
%
%If you wish to load the \verb+natbib+ package with options, you may
%add the following before loading the \verb+nips_2018+ package:
%\begin{verbatim}
%   \PassOptionsToPackage{options}{natbib}
%\end{verbatim}
%
%If \verb+natbib+ clashes with another package you load, you can add
%the optional argument \verb+nonatbib+ when loading the style file:
%\begin{verbatim}
%   \usepackage[nonatbib]{nips_2018}
%\end{verbatim}
%
%As submission is double blind, refer to your own published work in the
%third person. That is, use ``In the previous work of Jones et
%al.\ [4],'' not ``In our previous work [4].'' If you cite your other
%papers that are not widely available (e.g., a journal paper under
%review), use anonymous author names in the citation, e.g., an author
%of the form ``A.\ Anonymous.''
%
%\subsection{Footnotes}
%
%Footnotes should be used sparingly.  If you do require a footnote,
%indicate footnotes with a number\footnote{Sample of the first
%  footnote.} in the text. Place the footnotes at the bottom of the
%page on which they appear.  Precede the footnote with a horizontal
%rule of 2~inches (12~picas).
%
%Note that footnotes are properly typeset \emph{after} punctuation
%marks.\footnote{As in this example.}
%
%\subsection{Figures}
%
%\begin{figure}
%  \centering
%  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%  \caption{Sample figure caption.}
%\end{figure}
%
%All artwork must be neat, clean, and legible. Lines should be dark
%enough for purposes of reproduction. The figure number and caption
%always appear after the figure. Place one line space before the figure
%caption and one line space after the figure. The figure caption should
%be lower case (except for first word and proper nouns); figures are
%numbered consecutively.
%
%You may use color figures.  However, it is best for the figure
%captions and the paper body to be legible if the paper is printed in
%either black/white or in color.
%
%\subsection{Tables}
%
%All tables must be centered, neat, clean and legible.  The table
%number and title always appear before the table.  See
%Table~\ref{sample-table}.
%
%Place one line space before the table title, one line space after the
%table title, and one line space after the table. The table title must
%be lower case (except for first word and proper nouns); tables are
%numbered consecutively.
%
%Note that publication-quality tables \emph{do not contain vertical
%  rules.} We strongly suggest the use of the \verb+booktabs+ package,
%which allows for typesetting high-quality, professional tables:
%\begin{center}
%  \url{https://www.ctan.org/pkg/booktabs}
%\end{center}
%This package was used to typeset Table~\ref{sample-table}.
%
%\begin{table}
%  \caption{Sample table title}
%  \label{sample-table}
%  \centering
%  \begin{tabular}{lll}
%    \toprule
%    \multicolumn{2}{c}{Part}                   \\
%    \cmidrule(r){1-2}
%    Name     & Description     & Size ($\mu$m) \\
%    \midrule
%    Dendrite & Input terminal  & $\sim$100     \\
%    Axon     & Output terminal & $\sim$10      \\
%    Soma     & Cell body       & up to $10^6$  \\
%    \bottomrule
%  \end{tabular}
%\end{table}
%
%\section{Final instructions}
%
%Do not change any aspects of the formatting parameters in the style
%files.  In particular, do not modify the width or length of the
%rectangle the text should fit into, and do not change font sizes
%(except perhaps in the \textbf{References} section; see below). Please
%note that pages should be numbered.
%
%\section{Preparing PDF files}
%
%Please prepare submission files with paper size ``US Letter,'' and
%not, for example, ``A4.''
%
%Fonts were the main cause of problems in the past years. Your PDF file
%must only contain Type 1 or Embedded TrueType fonts. Here are a few
%instructions to achieve this.
%
%\begin{itemize}
%
%\item You should directly generate PDF files using \verb+pdflatex+.
%
%\item You can check which fonts a PDF files uses.  In Acrobat Reader,
%  select the menu Files$>$Document Properties$>$Fonts and select Show
%  All Fonts. You can also use the program \verb+pdffonts+ which comes
%  with \verb+xpdf+ and is available out-of-the-box on most Linux
%  machines.
%
%\item The IEEE has recommendations for generating PDF files whose
%  fonts are also acceptable for NIPS. Please see
%  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}
%
%\item \verb+xfig+ "patterned" shapes are implemented with bitmap
%  fonts.  Use "solid" shapes instead.
%
%\item The \verb+\bbold+ package almost always uses bitmap fonts.  You
%  should use the equivalent AMS Fonts:
%\begin{verbatim}
%   \usepackage{amsfonts}
%\end{verbatim}
%followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or
%\verb+\mathbb{C}+ for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You
%can also use the following workaround for reals, natural and complex:
%\begin{verbatim}
%   \newcommand{\RR}{I\!\!R} %real numbers
%   \newcommand{\Nat}{I\!\!N} %natural numbers
%   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
%\end{verbatim}
%Note that \verb+amsfonts+ is automatically loaded by the
%\verb+amssymb+ package.
%
%\end{itemize}
%
%If your file contains type 3 fonts or non embedded TrueType fonts, we
%will ask you to fix it.
%
%\subsection{Margins in \LaTeX{}}
%
%Most of the margin problems come from figures positioned by hand using
%\verb+\special+ or other commands. We suggest using the command
%\verb+\includegraphics+ from the \verb+graphicx+ package. Always
%specify the figure width as a multiple of the line width as in the
%example below:
%\begin{verbatim}
%   \usepackage[pdftex]{graphicx} ...
%   \includegraphics[width=0.8\linewidth]{myfile.pdf}
%\end{verbatim}
%See Section 4.4 in the graphics bundle documentation
%(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})
%
%A number of width problems arise when \LaTeX{} cannot properly
%hyphenate a line. Please give LaTeX hyphenation hints using the
%\verb+\-+ command when necessary.
%
%\subsubsection*{Acknowledgments}
%
%Use unnumbered third level headings for the acknowledgments. All
%acknowledgments go at the end of the paper. Do not include
%acknowledgments in the anonymized submission, only in the final paper.
%
%\section*{References}
%
%References follow the acknowledgments. Use unnumbered first-level
%heading for the references. Any choice of citation style is acceptable
%as long as you are consistent. It is permissible to reduce the font
%size to \verb+small+ (9 point) when listing the references. {\bf
%  Remember that you can use more than eight pages as long as the
%  additional pages contain \emph{only} cited references.}
%\medskip
%
%\small
%
%[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms
%for connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and
%T.K.\ Leen (eds.), {\it Advances in Neural Information Processing
%  Systems 7}, pp.\ 609--616. Cambridge, MA: MIT Press.
%
%[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS:
%  Exploring Realistic Neural Models with the GEneral NEural SImulation
%  System.}  New York: TELOS/Springer--Verlag.
%
%[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of
%learning and recall at excitatory recurrent synapses and cholinergic
%modulation in rat hippocampal region CA3. {\it Journal of
%  Neuroscience} {\bf 15}(7):5249-5262.

==> relatedwork.tex <==
\section{Related work}

Recent work by \citet{schoenholz2016deep} showed that an important factor responsible for reliable gradient flow during backpropagation is $\tilde{\chi} = \sigma^2_w \int \mathcal{D}_z\phi^{\prime}\left(\sqrt{\tilde{q}^*}z\right)^2$, which also happens to be related to the mean squared singular values of the input-output Jacobian $\mathbf{J} = \prod^L_{l=1} \textrm{diag}(\phi^\prime(\tilde{\mathbf{h}}^l))W^l$. Furthermore, during backpropagation, the expected magnitude of the gradient at each layer was shown to be proportional to the variance of its error vector $\tilde{\delta}^l$ and the following recursive variance relation was derived\footnote{An important note is that the derivation relies on the assumption that the weights used in the forward pass are sampled independently from those used during backpropagation.} 
\begin{align}
	\tilde{q}^l_\delta = \tilde{q}^{l+1}_\delta\frac{D_{l+1}}{D_l}\tilde{\chi},
	\label{eq: error variance relation}
\end{align}
where $\tilde{q}^l_\delta = \textrm{E}[(\tilde{\delta}^l_i)^2]$ with $\tilde{\delta}^l_i = \phi^\prime(\tilde{h}^l_i)\sum^{D_{l+1}}_{j=1}\tilde{\delta}^{l+1}_jW^{l+1}_{ji}$. For a network using ReLU activation $\int \mathcal{D}_z\phi^{\prime}\left(\sqrt{\tilde{q}^*}z\right)^2 = \int_0^\infty \mathcal{D}_z = \frac{1}{2}$, independent of the fixed point $\tilde{q}^*$ and therefore, $\tilde{\chi} = \frac{1}{2}\sigma^2_w$. In the case of constant width networks, the fixed point for \eqref{eq: error variance relation} requires that $\tilde{\chi} = 1$ such that $\sigma^2_w = 2$. However, critical initialization for multiplicative noise implies that $\tilde{\chi} = \frac{1}{2}\left(\sqrt{\frac{2}{\mu_2}}\right)^2 = \frac{1}{\mu_2}$. Therefore, to satisfy the relation in \eqref{eq: error variance relation}, the network architecture must adapt to the amount of noise injected into the network in such a way that the layer width $D_{l+1} = \mu_2D_l$. For example, in the case of dropout $D_{l+1} = D_l/p$, which implies that for any $p < 1$, each successive layer in the network needs to grow in width by a factor of $1/p$ to promote stable gradient flow. Similarly, for multiplicative Gaussian noise, $D_{l+1} = D_l(\sigma^2_\epsilon + 1)$, which requires the network to grow in width unless $\sigma^2_\epsilon = 0$.

\textcolor{red}{TODO: discuss experiments}

% The correlation dynamic for noisy neural networks are given by

% \begin{align}{}
% 	\tilde{q}^l_{ab} = \frac{1}{D_l}\sum^{D_l}_{j=1}\tilde{h}^l_j(\mathbf{x}^{0,a})\tilde{h}^l_j(\mathbf{x}^{0,b})
% \end{align}

% \begin{align}
% 	\tilde{q}^l_{ab} = \sigma^2_w\frac{1}{D_{l-1}}\sum^{D_{l-1}}_{j=1}\phi(\tilde{h}^{l-1}_j(\mathbf{x}^{0,a}))\phi(\tilde{h}^{l-1}_j(\mathbf{x}^{0,b})) + \sigma^2_b
% \end{align}
% Let $\tilde{\mathbf{x}}^{l-1, a} = \phi(\tilde{h}^{l-1}_j(\mathbf{x}^{0,a}))$, since the noise is sampled independently we then have that $\textrm{E}_\epsilon \left [ \tilde{\mathbf{x}}^{l-1, a} \cdot \tilde{\mathbf{x}}^{l-1, b} \right ] = \textrm{E}_\epsilon \left [ \tilde{\mathbf{x}}^{l-1, a} \right ] \cdot \textrm{E}_\epsilon \left [ \tilde{\mathbf{x}}^{l-1, b} \right ] = \mathbf{x}^{l-1, a} \cdot \mathbf{x}^{l-1, b}$. Using the result derived in \citep{poole2016exponential} we have

% \begin{align*}
% 	\tilde{q}^l_{ab} = \sigma^2_w \int \mathcal{D}_{z_1}\mathcal{D}_{z_2}\phi(\tilde{u}_1)\phi(\tilde{u}_2) + \sigma^2_b,
% \end{align*}
% where $\tilde{u}_1 = \sqrt{\tilde{q}^{l-1}_{aa}}z_1$ and $\tilde{u}_2 = \sqrt{\tilde{q}^{l-1}_{bb}}\left (\tilde{c}^{l-1}_{ab}z_1 + \sqrt{1-(\tilde{c}^{l-1}_{ab})^2}z_2 \right )$ with $\tilde{c}^l_{ab} = \frac{\tilde{q}^{l}_{ab}}{\sqrt{\tilde{q}^l_{aa}}\sqrt{\tilde{q}^l_{bb}}}$.


% Dynamical isometry in dropout rectifier networks

% In our case the mean squared singular value of the Jacobian is $\tilde{\chi}^L$, where 
% \begin{align}
% 	%\tilde{\chi} = \frac{\partial \tilde{c}^l_{ab}}{\partial \tilde{c}^{l-1}_{ab}} = \sigma^2_w \int \mathcal{D}_z\phi^{\prime}\left(\sqrt{\tilde{q}^*}z\right)^2
% 	\tilde{\chi} = \sigma^2_w \int \mathcal{D}_z\phi^{\prime}\left(\sqrt{\tilde{q}^*}z\right)^2
% 	\label{eq: chi}
% \end{align}
% thus we require that $\tilde{\chi} = 1$. For ReLU network $\int \mathcal{D}_z\phi^{\prime}\left(\sqrt{\tilde{q}^*}z\right)^2 = \int_0^\infty \mathcal{D}_z = \frac{1}{2}$, independent of the fixed point variance $\tilde{q}^*$. Therefore, $\chi = \frac{1}{2}\sigma^2_w$ which implies that $\sigma^2_w = 2$. 

% Furthermore, similar to ... it is relatively easy to show that if $\tilde{c}^{l-1}_{ab} = 1$ with $\tilde{q}_{aa} = \tilde{q}_{bb} = \tilde{q}^*$, then
% \begin{align*}
% 	\tilde{c}^l_{ab} & = \frac{\tilde{q}^l_{ab}}{\tilde{q}^*} \\
% 	& = \frac{1}{\tilde{q}^*}\left [ \sigma^2_w \int \mathcal{D}_z \phi(\sqrt{\tilde{q}^*}z)^2 + \sigma^2_b \right ] \\
% 	& = \frac{1}{\tilde{q}^*}\left [ \tilde{q}^* - \sigma^2_w\textrm{Var}(\tilde{\mathbf{x}}) \right ] \\
% 	& = 1 - \frac{\sigma^2_w\textrm{Var}(\tilde{\mathbf{x}})}{\tilde{q}^*},
% \end{align*}
% which in fact holds for any nonlinearity.

% For example, dropout satisfies the fixed point of recursive variance relation when $\sigma_w = \sqrt{2p}$, however this means that
% \begin{align*}
% 	\tilde{\chi} = \left (\sqrt{2p} \right)^2\frac{1}{2} = p
% \end{align*}
% which for any amount of dropout implies that $\chi < 1$.

\textcolor{red}{TODO: explain dynamical isometry}

Using tools of free probability \citet{pennington2017resurrecting} were able to derive the first two moments of the spectral density of $\mathbf{JJ}^T$ for a random constant width ReLU network as $m_1 = \left (\sigma^2_w/2 \right)^L$ and $m_2 = \left(\sigma^2_w/2\right)^{2L}(2L + 1)$. In our context, initializing at criticality for multiplicative noise distributions then gives the corresponding mean as $m_1 = (1/\mu_2)^L$, and variance as $\sigma^2_{JJ^T} = m_2 - m_1^2 = 2L\left(1/\mu_2 \right)^{2L}$. Therefore, for constant width, large depth noisy ReLU networks, the mean of the spectral density will either explode, or vanish, unless $\mu_2 = 1$. However, for all the common multiplicative noise distributions in Table \ref{tab: noise table}, any amount of noise results in $\mu_2 > 1$. For example, for dropout $\mu_2 = 1$ only if $1/p = 1$, which implies that $p=1$. For Gaussian noise it is required that $\sigma^2_\epsilon + 1 = 1$, such that $\sigma^2_\epsilon$ must be zero. Therefore noise, even at criticality, results in a vanishing mean. Similarly, $\sigma^2_{JJ^T}$ will also vanish for large $L$, when $\mu_2 > 1$.

==> signalprop.tex <==
\section{Signal propagation in deep neural networks}
\label{sec:signalprop}

We begin by providing a review of signal propagation in deep neural networks; we briefly describe the framework developed by \cite{poole2016exponential}, before extending it to our noisy setting in the next section.

Given input $\mathbf{x}^0 \in \mathbb{R}^{D_0}$, consider a deep neural network model with layer pre-activations specified by $\mathbf{h}^l = W^l\mathbf{x}^{l-1} + \mathbf{b}^l$, with weights $W^l \in \mathbb{R}^{D_l \times D_{l-1}}$, biases $\mathbf{b}^l \in \mathbb{R}^{D_l}$ and $D_l$ denoting the dimensionality of the $l^{th}$ hidden layer in the network.
The hidden layer activations $\mathbf{x}^l = \phi(\mathbf{h}^l)$ are computed element-wise using an activation function $\phi(\cdot)$, 
% with weights $W^l \in \mathbb{R}^{D_l \times D_{l-1}}$ and biases $\mathbf{b}^l \in \mathbb{R}^{D_l}$, 
for layers $l = 1, ..., L$.
% Here, $D_l$ denotes the dimensionality of the $l^{th}$ hidden layer in the network.
We consider the network behavior when the elements for the weights and biases are sampled i.i.d.\ from a zero mean Gaussian distribution with variances $\sigma^2_w/D_{l-1}$ and $\sigma^2_b$, respectively. In the large width limit, the empirical distribution of the pre-activations $\mathbf{h}^l$ can be treated as being Gaussian distributed with mean zero and variance $q^l = \sigma^2_w \mathbb{E}_z\left [ \phi\left(\sqrt{q^{l-1}}z \right)^2 \right ] + \sigma^2_b$ where $\mathbb{E}_z({z}) = \int\frac{1}{\sqrt{2\pi}}e^{-\frac{z^2}{2}}dz$ and the initial value $q^0 = \frac{1}{D_0}\mathbf{x}^0\cdot\mathbf{x}^0$. The recursive relation in~\eqref{eq: variance map} serves as an iterative variance map that can be used to compute the variance of the pre-activations at each layer. This map is displayed in Figure \ref{fig: noisy signal propagation} (a), for a network with tanh activation, $\phi(\mathbf{h}) = \textrm{tanh}(\mathbf{h})$ (yellow), as well as for ReLU activation, $\phi(\mathbf{h}) = \textrm{max}(0, \mathbf{h})$ (purple). 
\begin{figure}
 \includegraphics[width=\linewidth]{figs/add_noise_1.pdf}
		\caption{\textit{Deep signal propagation with and without noise}. Lines correspond to theoretical predictions and points to numerical simulations, for noiseless tanh (yellow) and noiseless ReLU (purple) networks, as well as for noisy tanh (red) and noisy ReLU (brown) networks with standard Gaussian noise. Both tanh networks use $(\sigma_w, \sigma_b) = (1,0)$ (``Xavier'' initialization), while the ReLU networks use $(\sigma_w, \sigma_b) = (\sqrt{2},0)$ (``He'' initialization). \textbf{(a)}:~Iterative variance map where the identity line is displayed as a dashed black line. \textbf{(b)}:~Variance dynamics during forward signal propagation.}
 \label{fig: noisy signal propagation}
\end{figure}
Solid lines show theoretical predictions from \eqref{eq: variance map} while points and shaded areas indicate means and standard deviations obtained from numerical simulations. (Details of the simulations are provided in the supplementary material.)
Note that the output variance for the tanh network (yellow) is bounded due to the saturating nature of the tanh activation function.
In contrast, for ReLU (purple), the activations are unbounded and therefore the output variance remains sensitive to the input variance at all levels.


To promote reliable signal propagation at initialisation for deep networks, it is useful for the pre-activations $\mathbf{h}^l$ to have roughly constant variance across layers during the first forward pass.
Without this property, the signal may either vanish or explode~\citep{poole2016exponential}.
If this leads to numerical issues such as floating-point overflow or underflow before the signal can reach the output layer (or during calculation of the loss function), the network may become untrainable.
In terms of \eqref{eq: variance map}, the constant variance fixed point is described as 
\begin{align}
	q^* = \sigma^2_w \int^\infty_{-\infty} \mathcal{D}_z \phi\left(\sqrt{q^*}z \right)^2 + \sigma^2_b.
	\label{eq: variance map fixed point}
\end{align}
In Figure \ref{fig: noisy signal propagation} (a), such a fixed point corresponds to a point situated on the identity line (black). Therefore, for an arbitrary activation function, a constant variance $q^*$ is achieved exactly points where its variance map intersects the identity line. For tanh networks, a fixed point always exists irrespective of the initialisation of the network.
However, for ReLU networks it can be shown that $(\sigma_w, \sigma_b) = (\sqrt{2}, 0)$, is the only critical initialisation that satisfies \eqref{eq: variance map fixed point}, referred to in this paper as the ``He'' initialisation \citep{he2015delving}, which is now often used. The variance dynamics for this initialisation are shown in green in Figure \ref{fig: noisy signal propagation} (b), displaying roughly constant behaviour.  

